TACAN: Transmitter Authentication through Covert Channels in Controller Area Networks

Nowadays, the interconnection of automotive systems with modern digital devices offers advanced user experiences to drivers. Electronic Control Units (ECUs) carry out a multitude of operations using the insecure Controller Area Network (CAN) bus in automotive Cyber-Physical Systems (CPSs). Therefore, dangerous attacks, such as disabling brakes, are possible and the safety of passengers is at risk. In this paper, we present TACAN (Transmitter Authentication in CAN), which provides secure authentication of ECUs by exploiting the covert channels without introducing CAN protocol modifications or traffic overheads (i.e., no extra bits or messages are used). TACAN turns upside-down the originally malicious concept of covert channels and exploits it to build an effective defensive technique that facilitates transmitter authentication via a trusted Monitor Node. TACAN consists of three different covert channels for ECU authentication: 1) Inter-Arrival Time (IAT)-based, leveraging the IATs of CAN messages; 2) offset-based, exploiting the clock offsets of CAN messages; 3) Least Significant Bit (LSB)-based, concealing authentication messages into the LSBs of normal CAN data. We implement the covert channels on the University of Washington (UW) EcoCAR testbed and evaluate their performance through extensive experiments. We demonstrate the feasibility of TACAN, highlighting no traffic overheads and attesting the regular functionality of ECUs. In particular, the bit error ratios are within 0.1% and 0.42% for the IAT-based and offset-based covert channels, respectively. Furthermore, the bit error ratio of the LSB-based covert channel is equal to that of a normal CAN bus, which is 3.1x10^-7%.

==> Sections/covert_channels.tex <==
\section{Covert Channels(3 Pages)}
\subsection{Timing Model}\label{sec:timing_model}
As illustrated in Fig.~\ref{fig:timing_model}, we let $t_i$ be the transmit time of message $i$ (assuming $t_0=0$) and $\Delta t_i = t_i - t_{i-1}$ be the inter-transmission time according to the transmitter's clock.
If messages are transmitted every $T$ sec, we have $\Delta t_i=T$ and $t_i=iT$. 
We consider the receiving ECU R's clock as the reference clock. 
In practice, there exists a clock skew in the transmitter's clock relative to the reference clock, which introduces an {\em offset} (time difference) $O_i$ between the two clocks. 
Therefore, the actual transmit time is $t'_i = t_i - O_i$. 
Given a clock skew $S$ \footnote{While the clock skew may be slowly varying subject to factors including the temperature, the clock skew is almost constant over  short durations.}, the relationship between the elapsed time $t_i$ at the transmitter and the elapsed time $t'_i$ at the receiver is given by $S = (t_i - t'_i)/t'_i$, and we have $O_i = \frac{S}{1+S} t_i$.
To account for offset deviations due to jitters at the transmitter, we model the actual clock offset $O_i = \frac{S}{1+S} t_i + \epsilon_i$, 
% \begin{equation*}
%     O_i = \frac{S}{1+S} t_i + \epsilon_i,
% \end{equation*}
where $\epsilon_i$'s are assumed to be i.i.d. zero-mean random variables.

\begin{figure}[t!]
\centering
\includegraphics[trim=0cm 0.9cm 0cm 0cm, clip=true, width=.9\columnwidth]{./Figures/timing_model}
\caption{Illustration of our timing model.}
\label{fig:timing_model}
\end{figure}

Affected by a network delay of $d_i$ (due to message transmission, propagation, arbitration, and reception) and the zero-mean quantization noise $n_i$ \cite{zander2008measurement}, the arrival timestamp of message $i$ is
\begin{align}
    a_i = t_i - O_i + d_i + n_i &=t_i - \frac{S}{1+S} t_i  + \eta_i =\frac{1}{1+S}t_i + \eta_i, \label{eq:arrival_timestamp}
\end{align}
where $\eta_i = -\epsilon_i + d_i + n_i$ is the overall noise term. 
Since periodic CAN messages have constant data lengths over time, it is reasonable to assume constant-mean network delays, i.e., $\mathbb{E}[d_i] = d$. 
Hence, $\eta_i$'s can be modeled as i.i.d. Gaussian random variables with $\eta_i \sim N(d, \sigma^2_\eta)$. 

\subsection{ITT-Based Covert Channel}
In the ITT-based covert channel, each ECU modifies (modulates) ITTs for transmitting its authentication bits, which can be observed (demodulated) by any receiver on the same bus. 
The key observation is that almost all CAN messages are periodically transmitted in automotive CAN, i.e., $\Delta t_i = t_i - t_{i-1}=T$, where $t_i$ is the transmit time of message $i$ and $T$ is the period.  
Hence, based on Eq.~(\ref{eq:arrival_timestamp}), the inter-arrival time (IAT) between messages $(i-1)$ and $i$ is
\begin{equation}
    \Delta a_i = a_i - a_{i-1} = \frac{1}{1+S} \Delta t_i + (\eta_i - \eta_{i-1}). \label{eq:inter_arrival_time}
\end{equation}
As a result, if the timing noise is small and the transmitter intentionally adjusts $\Delta t_i$ from $T$ to $(T+\delta)$ or $(T-\delta)$ to represent bits 0 or 1, respectively, where $\delta$ is a small fixed amount of deviation, the receiver will observe a corresponding change in $\Delta a_i$
%of $\delta/(1+S)$ (where the clock skew $S$ is usually very small) 
and demodulate the bits accordingly.
We now describe our observations of IATs and present our ITT-based covert channel.

\subsubsection{Observations.} 
Figure~\ref{fig:example_iat_distribution} provides the IAT distributions of an example message 0x020 ($T=0.01$) from the Toyota dataset \cite{toyota2010dataset}. 
To understand the effect of $\delta$, we add/subtract $\delta=0.02T=2\cdot 10^{-4}$ to/from the IATs\footnote{According to Eq.~(\ref{eq:inter_arrival_time}), with a change of $\delta$ in $\Delta t_i$, the corresponding change in $\Delta a_i$ would be $\delta/(1+S) \approx \delta$, since $S$ is very small (in the order of hundreds of ppm). }. 
As shown in Figure~\ref{fig:example_iat_distribution_L-1}, the three clusters centered at around $T$, $(T+\delta)$, and $(T-\delta)$ are overlapping with each other.
In this case, it is difficult to differentiate a bit 1 from a bit 0 (or from a silence bit) through thresholding, and the inter-cluster distance needs to be increased. 

While it is straightforward to increase $\delta$, there may be an upper limit $\delta_{\max}$ due to the real-time requirements of ECUs.
An alternative is to perform \textit{running average} to  smooth out the effect of noise.
Let the running averages of $\Delta a_i$'s with window length $L$ be $\Delta a_{i,L}$. 
As shown in Figure~\ref{fig:example_iat_distribution_L-3}, running averages can significantly reduce the variations due to noise and clearly separate the three clutsers from each other. 
In this example, the mean of averaged IATs is $0.01$.
With \textit{a lower threshold} $\Gamma_l=\mu(\Delta a,L)-\delta/2=0.0099$ and \textit{an upper threshold} $\Gamma_u=\mu(\Delta a, L)+\delta/2=0.0101$, the clusters can be distinguished from each other and bits can be determined accordingly. 
In general, to achieve completely non-overlapping clusters, $\delta$ and $L$ are chosen such that the following condition is met,
\begin{equation}
\delta > \max(\Delta a_{i,L})-\min(\Delta a_{i,L}), 
\end{equation}
where $\max(\Delta a_{i,L})$ and $\min(\Delta a_{i,L})$ 
are the minimum and maximum values of $\Delta a_{i,L}$, respectively.
Based on the above observations, we propose a ITT-based covert channel between a transmitter and a receiver without introducing any overhead, as described below.

\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[trim=0cm 0cm 1.3cm 1.3cm,clip=true,width=\textwidth]{Figures/example_iat_distribution_L-1}
        \caption{}
        \label{fig:example_iat_distribution_L-1}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[trim=0cm 0cm 1.3cm 1.3cm,clip=true,width=\textwidth]{Figures/example_iat_distribution_L-3}
        \caption{}
        \label{fig:example_iat_distribution_L-3}
    \end{subfigure}
    \caption{Example of IAT distributions of message 0x020 from the Toyota dataset (a) without running average and (b) with running average of $L=3$.}
    \label{fig:example_iat_distribution}
\end{figure}

\subsubsection{Embedding $A_s$ into ITTs}\label{sec:ITTM}
For each authentication sequence $A_s$, we first append a few silence bits ($\delta=0$) before and after $A_s$ to indicate the start and end of $A_s$. 
Then we modulate each bit $i$ into $L$ consecutive ITTs as follows,
\begin{equation}
    \Delta t_j =
    \begin{cases}
        T + \delta, & \text{ if } b_i = 0\\
        T - \delta, & \text{ if } b_i = 1\\
        T, & \text{ else }
    \end{cases},
    \text{ for } j \in [iL, (i+1)L).
\end{equation}
In other words, each bit is repeated $L$ times, including the silence bit.
We refer to the above scheme as \textit{ITT Modulation} (ITTM).

\subsubsection{Extracting $A_s$ from IATs}
In order to successfully establish the covert channel, the  parameters including $L$, $\Gamma_l$, and $\Gamma_u$ need to be shared between a transmitter and a receiver.
We assume that they are determined during manufacturing for given vehicle before entering the market.
We leave the blind estimation of the system parameters from the receiver side as future work.

One the receiver side, the receiver will filter for the targeted message, record arrival timestmaps, and compute inter-arrival times.
An example is provided in Figure~\ref{fig:example_running_average}, where $L=3$ and each $A_s=0101...01$ is $16$ bits long with $2$ silence bits before and after $A_s$.
As shown in Figure~\ref{fig:example_without_running_average}, without running average, the receiver will observe very large variations in IATs due to timing noise, which leads to many possible bit flitting. 
In contrast, by computing the running average with $L=3$, the receiver can effectively reduce the effect the noise. 
After sampling every $L$ IATs\footnote{We can see that the correct offset can be easily determined for each $A_s$ such that the total distance from each sample to the mean value of $(\Gamma_u+\Gamma_l)/2$ is maximized. }, the receiver can convert the sampled value $\Delta a[iL]$ into a bit as follows,
\begin{equation}
    \hat{b}_i =
    \begin{cases}
        0, & \text{ if } \Delta a[iL] > \Gamma_u\\
        1  & \text{ if } \Delta a[iL] < \Gamma_l\\
        NULL, & \text{ else  // (Silence bit) }
    \end{cases}.
\end{equation}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[trim=0cm 0cm 1.3cm 1.3cm,clip=true,width=\textwidth]{Figures/example_without_running_average}
        \caption{}
        \label{fig:example_without_running_average}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[trim=0cm 0cm 1.3cm 1.3cm,clip=true,width=\textwidth]{Figures/example_with_running_average}
        \caption{}
        \label{fig:example_with_running_average}
    \end{subfigure}
    \caption{Example of observed IATs at the receiver side (a) without and (b) with running average of $L=3$.}
    \label{fig:example_running_average}
\end{figure}

% \cmt{How to deal with missing message? Include the discussion in the appendix.}

% \begin{figure}[t!]
% 	\centering
% 	\begin{subfigure}[h]{1\columnwidth} % {0.48\columnwidth}
% 		\includegraphics[width=\columnwidth]{./Figures/tx_normal}
% 		\caption{Inter-transmission times without any embedding}
% 		\label{fig:tx_normal}
% 	\end{subfigure}
% 	\begin{subfigure}[h]{1\columnwidth} % {0.48\columnwidth}
% 		\includegraphics[trim={0 0.5cm 0 0},clip,width=\columnwidth]{./Figures/tx_delay_embedding}
% 		\caption{Delay-embedding inter-transmission times}
% 		\label{fig:tx_delay_embedding}
% 	\end{subfigure}
% 	\begin{subfigure}[h]{1\columnwidth} % {0.48\columnwidth}
% 		\includegraphics[trim={0 0.5cm 0 0},clip,width=\columnwidth]{./Figures/tx_msg_count_embedding}
% 		\caption{Message-count-embedding inter-transmission times}
% 		\label{fig:tx_msg_count_embedding}
% 	\end{subfigure}
% 	\begin{subfigure}[h]{1\columnwidth} % {0.48\columnwidth}
% 		\includegraphics[trim={0 0.5cm 0 0},clip,width=\columnwidth]{./Figures/tx_hybrid_embedding}
% 		\caption{Hybrid-embedding inter-transmission times}
% 		\label{fig:tx_hybrid_embedding}
% 	\end{subfigure}
% 	\caption{Embedding techniques }
% \end{figure}


% \shaun{Metrics: 1) throughput, 2) bit error (robustness), 3) efficiency response time (i.e., time it takes to detect anomalies), 4) effectiveness -- detection rate }

% Things to consider: 1) Noise, 2) missing messages in normal cases. 

% \subsection{Order-Based Covert Channel}
% An ECU may transmit multiple messages consecutively. By adjusting the order of transmitted messaegs, the ECU can also embed authentication bits. 
% For example, if the ECU is transmitting two messages X,Y, then transmitting message X followed by message Y represents a bit 0 and otherwise a bit 1. 
% If the ECU is transmitting three messages X, Y, and Z, then there are a total of 6 different combinations, which can represent $\log_2(6) \approx 2.58$ bits. 

% Note that the mapping table can be assumed to be known. 

\subsection{Offset-Based Covert Channel}
As the CAN bus load increases, the noise in ITTs caused by arbitration can be very significant, which may require a large $\delta$ value to establish a reliable ITT-based covert channel, at the risk of violating possible real-time requirements. 
In the offset-based covert channel, the receiver computes the offset in order to accumulate the deviations that carry the authentication information, instead of averaging them (through running average). 
In the rest of this section, we will explain the concept of clock offset and present our offset-based covert channel scheme in detail. 

% On CAN buses with heavy traffic, the noise in ITTs caused byarbitration can be very significant, and it would require a largeδvalue in order to establish a reliable ITT-based covert channel.Taking the message with ID=0x0C5 andT=10ms in the EcoCAR[1] as an example

% \begin{figure}[ht!]
%     \centering
%     \begin{subfigure}[b]{0.48\columnwidth}
%         \includegraphics[trim=0cm 0cm 1.3cm 1.3cm,clip=true,width=\textwidth]{Figures/example_offset_based_CC_0c5_IATs}
%         \caption{}
%         \label{fig:example_offset_based_CC_0c5_IATs}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[b]{0.48\columnwidth}
%         \includegraphics[trim=0cm 0cm 1.3cm 1.3cm,clip=true,width=\textwidth]{Figures/example_offset_based_CC_0c5_offsets}
%         \caption{}
%         \label{fig:example_offset_based_CC_0c5_offsets}
%     \end{subfigure}
%     \caption{Example message with ID=0x0C5 and a period of $T=10$ ms from the EcoCAR \cite{ecocar}. (a) The IATs vary between $9.3$ ms and $10.7$ ms. (b) Accumulated offsets. }
%     \label{fig:example_offset_based_CC_0c5}
% \end{figure}


\subsubsection{Observations}
According to our timing model for arrival timestamps in Eq.~(\ref{eq:arrival_timestamp}), we have
\begin{equation}
    a_i - a_0 = \left(t_i - \frac{S}{1+S}t_i + \eta_i \right) - \eta_0. \nonumber
\end{equation}
Then the observed clock offset is given by
\begin{equation}
    \hat{O}_i = t_i - (a_i-a_0) = \frac{S}{1+S} t_i + r_i = \frac{S}{1+S} \sum_{j=1}^{i} \Delta t_j + r_i, \nonumber
\end{equation}
where $r_i = \eta_0 - \eta_i$ is the zero-mean residual.  
Since $\Delta t_j = T$ for periodic CAN messages, the residual becomes
\begin{equation}
    r_i = \hat{O}_i - \frac{S}{1+S} \cdot iT \nonumber
\end{equation}
If the transmitter adds a deviation of $\delta$ to $L$ consecutive ITTs while keeping others the same (i.e., $\Delta t_j = T+\delta$ for $j=1, ..., L$), the resulting residual is
\begin{equation}
    r'_i = \hat{O}_i - \frac{S}{1+S} \cdot (iT + \delta L) = r_i - \frac{S}{1+S} \cdot \delta L. \nonumber
\end{equation}
As we can see, the effect of adding deviations will accumulate and manifests itself in the clock offset (and its residual).  
By detecting the change in clock offsets, the receiver can demodulate the authentication sequences. 
In what follows, we will explain our offset-based covert channel in more detail. 

\subsubsection{Embedding $A_s$ into Offsets}
Unlike the ITTM scheme (Section~\ref{sec:ITTM}), we modulate each bit into $L$ consecutive ITTs as follows,
\begin{equation}
    \Delta t_j =
    \begin{cases}
        T + \delta, & \text{ if } b_i = 0\\
        T - \delta, & \text{ if } b_i = 1\\
        T, & \text{ else }
    \end{cases},
    \text{ for } j \in [iL, iL+L/2),
\end{equation}
and 
\begin{equation}
    \Delta t_j =
    \begin{cases}
        T - \delta, & \text{ if } b_i = 0\\
        T + \delta, & \text{ if } b_i = 1\\
        T, & \text{ else }
    \end{cases},
    \text{ for } j \in [iL+L/2, (i+1)L),
\end{equation}
where $L$ is assumed to be an even integer. 
In other words, we add/subtract $\delta$ to/from $T$ for the first $L/2$ ITTs and subtract/add $\delta$ for the next $L/2$ ITTs to maintain the baseline of clock offsets.


\subsubsection{Extracting $A_s$ from Offsets}
On the receiver side, arrival timestamps are processed in batch. 
For each batch, update the clock skew estimate at the beginning of each batch (during the transmission of silence bits). 
Then use the updated clock skew to compute the clock skew residuals for that batch. 
Thresholding: find the mid-point ((min+max)/2); the upper threshold is mid-point + $\delta$*L/4; the lower threshold is mid-point - $\delta$*L/4. 
Finally, sample at every $L$ points (with the correct offset) and convert the sampled values to bits. 


\subsection{Storage-Based Covert Channel}

\begin{itemize}
    \item [1] using Data Frame and Base frame format (with 11 identifier bits);
    \item [2] using least significant bit of Data Field $d_f$ (0-8 bytes) to carry the secret message;
    \item [3] monitor node (IDS) and ECU $i$ know the pre-shared key $K_{s_i}$ (secret message);
    \item [4] binary pre-shared key $K_{s_i}$ is constituted of $n$ bits
    \item [5] sync btw ECU $i$ and Monitor node to start Key transmission \hl{(how to sync ECU and Monitor node to start the Key transmission?)}
    \item [6] ECU $i$ starts to send $K_{s_i}$ most significant bit $K_{s_i}[0]$ including it in the least significant bit of $d_f$ according to the following equations:
\begin{equation}
    value(d_f) =
	\begin{cases}
      value(d_f) & if K_{s_i}[0] = bin(d_f(least\_sign\_bit))\\
      value(d_f) + \gamma & if K_{s_i}[0] \neq bin(d_f(least\_sign\_bit))
   \end{cases}
\end{equation}
    where:
\begin{equation}
    \gamma = min(value(\cdot)) \mid bin(d_f(least\_sign\_bit)) + \gamma = K_{s_i}[0]
\end{equation}

\giuseppe{Example: consider the value of the temperature in the $d_f$ and the IEEE-754 Floating Point conversion schema: 45.84 degrees Celsius is 01000010001101110101110000101001 in binary representation while 45.85 degrees Celsius is 01000010001101110110011001100110. As you can see, a very small difference allows to transmit 0 or 1 as a least significant bit.}

\shaun{Find a real example in CAN traffic}

    \item [7] following $K_{s_i}[i]$, $i \in \{1,...,n\}$ bits are transmitted according to the same rule explained in (6)
    
    \item \hl{point of attention: Cyclic Redundancy Check (CRC) for the CAN frame needs to be computed after the eventual bit modification.}

    \item \hl{point of attention: we could consider to extend the trasmission using more than a single bit, such as using the last three bits of the $d_f$ cons: value changed will be greater}

\end{itemize}

\shaun{Can be used to transmit both key and authentication bits.}

\giuseppe{do we still need the following itemize?}
Covert Channel for authentication proposed methodology description:
\begin{itemize}
    \item Time-based CC based on Clock Skew for authentication in CAN.
    \item Storage-based CC based on least significant bit in CAN communication between ECU and Monitoring node (i.e., IDS).
\end{itemize}

\hl{We could combine the two methodologies to better address authentication requirements, such as synchronization for the communication of the secret message used for the authentication.}

==> Sections/protocol.tex <==
\section{Transmitter Authentication Protocol (1 Page)}
In this section, we present our transmitter authentication protocol.

%and three covert channels for transmitting authentication sequences: 1) inter-transmission time (ITT)-based covert channel, 2) offset-based covert channel, and 3) least-significant-bit (LSB)-based covert channel.  

%\subsection{Transmitter Authentication Protocol}
\subsubsection{Key Exchange} 
There is a pre-shared key (or program/code) stored in tamper-proof storage. 
Need a protocol that generates session keys. 

\subsubsection{Transmitter Authentication}
Each ECU $i$ keeps a counter $c_i$ that counts for the number of authentication messages that have been transmitted. 
The use of a counter aims to prevent replay attacks.
The authentication sequence is 
\begin{equation}
    A_s = c_i || HMAC(K_{s_i}, c_i),
\end{equation}
where $K_{s_i}$ is the session key for ECU $i$ and HMAC refers to the hash-based message authentication code algorithm.
Since digests are usually of hundreds of bits (e.g., SHA-1's digests are 160 bits and SHA-256's digests) that is too long due to low authentication bit rate, we may truncate each MAC to 8 bits or XOR all MAC bytes together to create a condensed 8-bit version of the MAC. 
If the counter is 24-bit long, then each authentication sequence is 32 bits (4 bytes). 

\begin{itemize}
    \item Do we need additional error-correcting code? Start of frame, end of frame? 
    \item Is this scheme secure?
    \item Do we need nonce? 
    \item If there is only counter, the receiver can verify the bits on the fly? 
    \item The counter reaches the maximum value, a new session key needs to be generated. 
    \item Depending on the time it takes to transmit one authentication sequence, the total duration of a valid session key can be very long. 
\end{itemize}

\textbf{Message-based counter. } 
Prevent a reply attack. Two counters may be out of sync due to network fault, which needs to be dealt with appropriately \cite{lin2012cyber}. 


==> Sections/system_model.tex <==
\section{System Model (0.5 page)}
Assumptions:
\begin{itemize}
    \item Each ECU has a shared secret (key) with the monitoring node (i.e., IDS). 
    \item Since the CAN bus is a broadcast medium, the adversary has access to all the data that is transmitted on the  bus. 
    \item The adversary does not have access to the tamper-proof storage.
\end{itemize}

\subsection{Clock-Related Definitions}


\begin{figure}[t!]
\centering
\includegraphics[width=.9\columnwidth]{./Figures/timing_model}
\caption{Timing model of message arrivals on the CAN bus.}
\label{fig:timing_model}
\end{figure}

\subsection{Timing Model}
Fig.~\ref{fig:timing_model} illustrates our timing model. 
We consider the clock of the receiving ECU R (the monitor node) as the reference clock. 
For illustration, let us consider an ECU that transmits messages every $T$ seconds. 
In the case where the transmitter's clock and the receiver's clock are synchronized, the $i$-th message will be transmitted at $t_i=iT$. 
In practice, however, there exists an {\em offset} (time difference) $O_i$ between the transmitter's clock and the receiver's due to the existence of the clock skew, and the actual transmit time is $t'_i = t_i - O_i$. 

According to Eq. XX, the relationship between the clock skew $S$, the elapsed time $t_i$ at the transmitter, and the elapsed time $t'_i$ at the receiver is given by $S = (t_i - t'_i)/t'_i$ and we have $O_i = \frac{S}{1+S} t_i$.
Since that $O_i$ is accumulating over time, we often refer to it as the accumulated offset. 
Note that while the clock skew may be slowly varying subject to factors including the temperature, the clock skew is usually constant over a short duration \cite{?}. 
To further account for offset deviations due to jitters at the transmitter, we model the actual clock offset as a random variable $O_i = \frac{S}{1+S} t_i + \epsilon_i$, where the $\epsilon_i$'s are assumed to be independent and identically distributed zero-mean random variables. 

After a network delay of $d_i$ (due to message transmission, propagation, arbitration, and reception), the arrival timestamp of the $i$-th message is given by
\begin{equation}
    a_i=t_i - O_i + d_i + n_i=\frac{1}{1+S}t_i - \epsilon_i + d_i + n_i,
\end{equation}
where $n_i$ is the quantization noise with a zero mean \cite{?}. 

Let $\eta_i = -\epsilon_i + d_i + n_i$. 
Since a CAN message usually has a fixed data length and ID, it is reasonable to assume constant-mean network delays, i.e., $\mathbb{E}[d_i] = d$.
Therefore, we model the $\eta_i$'s as i.i.d. Gaussian random variables with $\eta_i \sim N(d, \sigma_\eta^2)$. 
In addition, the inter-arrival time $\Delta a_i$ between messages $(i-1)$ and $i$ is given by
\begin{equation}
    \Delta a_i = a_i - a_{i-1} = \frac{1}{1+S} \Delta t_i + (\eta_i - \eta_{i-1}),
\end{equation}
where $\Delta t_i = t_i - t_{i-1}=T$ is the inter-transmission time as per the transmitter's local clock. 
Hence, the mean of the inter-arrival times is $\mu \triangleq \mathbb{E}[\Delta a_i] = \frac{1}{1+S} t_i$ and its variance is $\sigma^2 \triangleq Var(\Delta a_i) = 2\sigma_\eta^2$. 

\subsection{Adversary Model}
\begin{itemize}
    \item Existing ECUs are compromised
    \item Adversary nodes are connected to the bus. 
\end{itemize}

Fabrication attacks, suspension attacks, and masquerade attacks, bus-off attacks. \giuseppe{MITM?}


\begin{figure}[t!]
\centering
\includegraphics[width=1\columnwidth]{./Figures/cc_schemas}
\caption{Covert channels schemas to transmit authentication messages.}
\label{fig:cc_schemas}
\end{figure}
